Improving Generalization of Transfer Learning Across Domains Using Spatio-Temporal Features in Autonomous Driving

Practical learning-based autonomous driving models must be capable of generalizing learned behaviors from simulated to real domains, and from training data to unseen domains with unusual image properties. In this paper, we investigate transfer learning methods that achieve robustness to domain shifts by taking advantage of the invariance of spatio-temporal features across domains. In this paper, we propose a transfer learning method to improve generalization across domains via transfer of spatio-temporal features and salient data augmentation. Our model uses a CNN-LSTM network with Inception modules for image feature extraction. Our method runs in two phases: Phase 1 involves training on source domain data, while Phase 2 performs training on target domain data that has been supplemented by feature maps generated using the Phase 1 model. Our model significantly improves performance in unseen test cases for both simulation-to-simulation transfer as well as simulation-to-real transfer by up to +37.3\% in test accuracy and up to +40.8\% in steering angle prediction, compared to other SOTA methods across multiple datasets.

==> sections/ablation.tex <==
\section{Selection of Visual Elements in Driving}
\newcommand\pN{\mathcal{N}}
\label{sec:ablation}
%\textbf{Laura: Needs to be edited so that it succinctly tells information. Looks like an information dump at the moment, needs some reorganizing.}

The dynamics and geometry of visual elements should remain constant across virtual and real domains. The vehicle will still follow the same constructs of driving behavior: staying between road markings, turning and rotating around a vertical axes, etc. We study the significance of key visual elements by observing the change in model parameters over image sequences, measured with cosine similarity. 

% We study the significance of the key factors in decision making through an ablation study. We first measure the cosine similarity in latent representations of each factor across image frames in a sequence. Cosine similarity is used as a distance metric between latent features representations of different images to understand how changes in an image sequence over time affect the learning output. We incorporate this into a novel transfer learning framework by complementing data with gradients and edge maps alongside sequential data. Our results show to generalize better across domains in Section~\ref{sec:methodology}.
% We explore several components of driving by isolating specific image sequences and extracting their hidden state representation during the learning process. 
% By taking the cosine similarity between latent feature representations, we can observe how visual and temporal changes across image sequences, such as rotation, affect change in the feature level representation in during learning. 

\vspace*{0.5em}
\noindent
\textbf{Studied Elements. } We study five different elements to empirically determine their contribution to decision making in driving. These five components are listed below. 

\begin{enumerate}
    \item \textbf{Projected distance}: the distance (in meters) from nearby vehicles, studied in Table~\ref{tab:ablation-distance}.
    \item \textbf{Vehicle rotation}:  the rotation at which a vehicle is performing at any given moment.
    \item \textbf{Optical flow}: motion flow of objects/pixels in a scene.
    \item \textbf{Gradient information}:  change in pixel values, analogous to edge detection, studied in Table~\ref{tab:ablation-gradient}.
    \item \textbf{Moving Objects}: dynamic obstacles in the scene.
\end{enumerate}

\noindent
While the first three of these capture the states of a  dynamical  system,  
the  last two characterize the geometry of the surrounding environment and other objects in the scene. Projected distance, vehicle rotation, and dynamic obstacles can be tangibly observed, while optical flow and gradient information are elements that are inferred by the model during learning. 

\subsection{Comparison of Image Similarity Metrics} 
% Common image similarity or distance metrics capture image similarity on a global statistical level or at a pixel level, typically not on a semantic pairwise level.
We use the cosine similarity to measure the closeness in image feature representations during the learning process, and compare its ability to correlate to collision confidence with Frechet Inception Distance (FID) and Structural Similarity Index Measure (SSIM).

Frechet Inception Distance~\cite{fid-metric} measures the distance between two datasets by comparing the mean and standard deviation of the activations in an Inception network. We calculate the FID using~\cite{Seitzer2020FID} in our observations. 
% The Frechet Inception Distance is formulated below for image distributions $X$ and $Y$, where $X,Y \sim \pN(\mu,\sum)$ and $Tr()$ is the scalar sum of diagonals in a matrix. 
% \vspace*{-1em}
% \begin{align*}
%     FID(X,Y) &= ||\mu_X - \mu_Y||^2_2 \\
%     &+ Tr\left(\textstyle \sum_X + \sum_Y  - 2 \left(\sum_X\sum_Y\right)^{\frac{1}{2}}\right)
% \end{align*}
While FID is powerful and standard for measuring the quality of images synthesized by generative adversarial networks (GANs), it is typically used to measure the distance between two image distributions. In our use case, we are interested in measuring the distance between model parameters upon input images of same (similar) distribution at different points in time.  Thus, FID measurements would not be appropriate. 

Another metric we consider is the SSIM ~\cite{ssim-metric}, a perception-based metric primarily used for assessing image quality. 
SSIM is robust to various transformations and is commonly used in image quality assessments; but it considers pixel-level representations of images, and not semantic representations in learning. This is a stark difference from FID, which is farther from pixel-level representation and closer to learned perception. 

% SSIM takes into account three components when comparing images: luminance $l$, contrast $c$, and structure $s$. The full calculation of SSIM is shown below for two individual images $x$ and $y$, with pixel-value mean $\mu$, covariance $\sigma$, constants $c$ for stabilization, and weights $\alpha$, $\beta$, and $\gamma$.

% \begin{align*}
%     l(x,y) &= \frac{2\mu_x\mu_y + c_1}{\mu_x^2 + \mu_y^2 + c_1} \\
%     c(x,y) &= \frac{2\sigma_x\sigma_y + c_2}{\sigma_x^2 + \sigma_y^2 + c_2} \\
%     s(x,y) &= \frac{\sigma_{xy} + c_3}{\sigma_x\sigma_y + c_3} \\
%     SSIM(x,y) &= \left[l(x,y)^\alpha \cdot c(x,y)^\beta \cdot s(x,y)^\gamma \right]
% \end{align*}

\begin{figure}[ht]
    \centering
     \vspace*{-0.5em}
    \includegraphics[width=7cm]{imgs/cosine-computation.png}
    \vspace*{-1em}
    \caption{Method for computing cosine similarity measurements in the ablation study. Reference sequences include base driving images, while target (test) sequences include saliency, gradient, and edge maps. Cosine similarity is computed from feature vectors extracted from intermediary layers of the CNN+LSTM network. Greater similarity measurements (closer to 1) indicate closeness in model perception of the data. }
    \vspace*{-1.5em}
    \label{fig:control-system}
\end{figure}

Since the focus of our study is to measure the impact of visual components on learning, we require a metric that can also consider the features of the network closer to learned perception, similarly to FID, but on a pairwise basis, where images may be from the same distribution, like the SSIM. We propose using cosine distance between vectors of LSTM hidden layer features $x$ and $y$ formulated as: \\

\vspace*{-2em}
\begin{align*}
 similarity(x,y) &= \frac{x \cdot y}{||x|| ||y||}
\end{align*}
\noindent
$x$ and $y$ are 32-dimensional vectors that represent hidden  state  features (i.e. model parameters or weights) extracted from the CNN+LSTM network, for both image sequences.
An advantage of cosine similarity over other metrics for comparing vectors, such as Euclidean distance, is that cosine similarity normalizes the magnitude of the vector, not letting
the magnitude of the vector or the dimensionality of the data affect the similarity 
measurement. % For high-dimensional data such as text documents or images, this avoids the Curse of Dimensionality. 
We show quantitative comparison among the three metrics in Tables~\ref{tab:ablation-distance} and ~\ref{tab:ablation-gradient}.

% \vspace*{0.5em}
% \noindent
\subsection{Measurement Methodology} 
% To measure the impact of each of the five driving elements, we choose chronological sequences of images from image data that are heavily representative of each factor over time. 
% For example, to study projected distance, we will choose sequences of data in which change in other factors like vehicle rotation, optical flow, and dynamic objects is minimal and the change in distance to other vehicles is apparent or emphasized. 
% We obtain the vectors for use in cosine similarity by first training a CNN+LSTM network on a simple binary classification task of ``safe'' versus ``dangerous'' scenarios. For each element, we define a set of reference images that represent the safe label at a high confidence for the classifier. Then, we increment the intensity of each element across different levels. 
We choose image sequences in which each of the five visual elements named are observed over time. For example, a sequence featuring a change in projected distance may include a vehicle moving closer or farther from the camera. Model representations of the images are obtained from inference of the fully trained network following phase two of transfer learning. 
We measure four levels of changes in metrics for projected distance, with level 1 being the smallest change in projected distance over time and level 4 being the largest change.
Since the learning task is binary classification of ``safe" versus ``collision", we expect there to be greater change in measured cosine similarity as collision confidence (i.e. the probability of predicted collision by the model) changes. Intuitively, as nearby vehicles become closer past a certain threshold, the collision confidence will greatly increase. See comparison for projected distance in Table~\ref{tab:ablation-distance}. 

% \textbf{mention how we measure collision confidence? Is it a metric that is given to us by CARLA?}

\begin{table}[h!]
    \centering
    \begin{tabular}{c c c c c c}
    \toprule
        Seq & $m$ & \textbf{Cosine} & FID & SSIM & Confidence(\%)\\ 
        \midrule
        %Ref & 92 & \textbf{1} & 0 & 1 & 0.8\\ 
        Level1 & 65 & \textbf{0.881} & 158.326 & 0.511 & 1.2\\
        Level2 & 45 & \textbf{0.781} & 237.496 & 0.439 & 5.4\\
        Level3 & 18 & \textbf{0.350} & 258.921 & 0.513 & 10.2\\
        Level4 &  4 & \textbf{0.286} & 237.108 & 0.415 & 81.6\\
    \bottomrule
    \end{tabular}
    \caption{Quantitative study of cosine similarity trends over changes in \textbf{projected distance} in $m$ meters. {\em As projected distance decreases and the objects come closer, the classifier's confidence of ``collision'' becomes significantly higher. As the collision confidence increases, the cosine similarity decreases since cosine similarity should correspond to confidence in the ``safe'' classification, which is noticeable here}. On the contrary, FID and SSIM show inconsistent trends with respect to collision confidence. }
    % Closer the nearby vehicle in a driving scenario, more the weightage of the projected distance in the AI decision making.
    % We observe that as the projected distance of nearby vehicles decreases, the spatio-temporal embeddings become less similar to the 'non-collision' reference scenario and the chances of collision increases exponentially}
    
    %Measurement of \textbf{projected distance z (m)} using similarity between hidden LSTM states. In a collision recognition binary classification task, we expect from human experience that distance to nearby vehicles plays a large role in evaluating the safety of a situation. Here, smaller gaps between nearby vehicles greatly affects the state of the LSTM in decision making, showing that projected distance quantitatively plays a significant role in decision making.}
    \label{tab:ablation-distance}
    \vspace*{-3em}
\end{table}

In addition, we observe the differences in learning perception of the base dataset and its gradient and saliency maps, which are measured similarly to projected distance above. We sample three different image sequences for GradCAM~\cite{gradcam} and Vanilla Gradient~\cite{vanilla-gradient}, where collision confidence is equal.
We do this to measure the difference in model-level perception of raw image data versus information presented by gradient and saliency maps. The base image sequences represent original data from CARLA Town 1. We compare these to the gradient and saliency maps produced by the same dataset, with samples taken from locations with same collision confidence. See comparison in Table~\ref{tab:ablation-gradient}. 

\begin{table}[h!]
\vspace*{0.5em}
    \centering
    \begin{tabular}{c|c c c c c}
    \toprule
        Seq & Technique & \textbf{Cosine} & FID & SSIM & Confidence(\%)\\
        \midrule
        %Ref & None & \textbf{1} & 0 & 1 & \\ 
        1 & Grad-CAM  & \textbf{0.635} & 512.73 & 0.0703 & 1.2\\
        1 & Vanilla & \textbf{0.635} & 698.98 & 0.0576 & 1.2\\
        2 & Grad-CAM  & \textbf{0.568} & 493.94 & 0.0733 & 1.2\\
        2 & Vanilla & \textbf{0.624} & 632.77 & 0.0557 & 1.2\\
        3 & Grad-CAM  & \textbf{0.632} & 403.62 & 0.0654 & 1.2\\
        3 & Vanilla & \textbf{0.633} & 403.62 & 0.0654 & 1.2\\
        \midrule
         & Both & \textbf{0.0424} & 0.2296 & 0.1067 \\
        $\widetilde{\sigma}$ & Grad-CAM & 0.0619 & 0.1240 & \textbf{0.0572} & -\\
        & Vanilla & \textbf{0.0093} & 0.2679 & 0.0863\\
    \bottomrule
    \end{tabular}
    \caption{Quantitative study of cosine similarity metric in relation to \textbf{ gradient visualization} data.  We study two gradient techniques, Grad-CAM~\cite{gradcam} and Vanilla backpropagation~\cite{vanilla-gradient}, across three different image sequences (involving scenario of the agent moving in with nearby vehicles) with equivalent classification confidence for ``collision''.  {\em The cosine similarity shows consistent and constant results, i.e. a low standard deviation across different images with similar classification confidence.} For FID and SSIM, we observe that normalized standard deviation $\widetilde{\sigma}$ (i.e. $\sigma/\mu$) is higher, and thus less reliable in measuring classifier confidence in learning. }
    %We observe that the cosine weightage vary about a mean of around 62 percent and there exists a constant relationship with the collision probablity}
    
    %Higher the relative velocity between the objects/vehicles/pedestrians and the agent, more is it's weightage in the AI decision making.We use image editing tools to segment moving objects of our test cases from our references.Note that the test cases contain only the segmented dynamic object from the references.We extract the spatio-temporal feature embeddings of reference scenarios and calculate its similarity from the respective test case embeddings. We observe that the weightage is within the range of 10-15 percent with slight increase  with increasing velocity}
    \label{tab:ablation-gradient}
    \vspace*{-1.5em}
\end{table}

These studies serve the purpose of validating cosine similarity as a suitable metric in analyzing its impact on decision making for driving, compared to two other well-known metrics. Next we use mean cosine similarity to measure the similarity between model perception of base image data and gradient/saliency maps for different scenarios using each one of the five spatio-temporal visual elements mentioned above. % projected distance, vehicle rotation, optical flow, gradient information, and dynamic obstacles.  
We observe these five global spatio-temporal features account for around a total
contribution of 78\% in the latent representations of the network, as shown in Table~\ref{tab:scenarios}.


% ADD THIS TO THE APPENDIX
 \begin{table}[ht]
     \centering
     \begin{tabular}{c|c c  }
     \toprule
         Seq & Spatio-Temporal features & Mean Significance (\%) \\
         \midrule
         %Ref & - & \textbf{1} & 0 & 1\\ 
         1 & Optical Flow  & \textbf{46} \\
         2 & Rotational Component  & \textbf{28} \\
         3 & Gradients & \textbf{64} \\
         4 & Moving cars and dynamic obstacles & \textbf{16} \\
         \midrule
         $\mu$ & All Together &  \textbf{78}\\
         %3 & 5 & \textbf{0.1563} & &\\
     \bottomrule
     \end{tabular}
     \caption{Quantitative analysis of the mean contribution in percentage of the global spatio-temporal features (including optical flow, agent's orientation, spatial gradients across frames, and dynamic obstacles) in the networks decision making. We observe these features together account for around 78\% contribution in the overall decision making of the network.}

     \label{tab:scenarios}
     \vspace*{-3em}
 \end{table}


% When measuring cosine similarity, we consider two sets of image sequences, namely a reference sequence and a target sequence. A reference sequence contains unprocessed images. A target sequence is defined as a sequence of images in which the studied factor is being observed, as shown in Figure~\ref{fig:control-system}. For example, in projected distance, the target sequence is a series of images where the distance to the nearby vehicles decreases with time. We observe the changes in cosine similarity over these changes in time. When passing these sequences through the classifier, we extract the hidden state vectors of the LSTM that correspond to these images we pass. Hidden state vectors in our network are 32 dimensional vectors. The dimensional size of 32 is a hyperparameter we defined for our network when training on the end-to-end classification task. 
% We observed better accuracy for our model using 32-dimensional hidden state vectors.   
% Cosine similarity is then measured between the hidden state vectors corresponding to the reference sequence and test (target) sequences respectively. 
% Due to limited space, we have included only the studies on projected distance and gradient elements in Tables~\ref{tab:ablation-distance} and~\ref{tab:ablation-gradient}, respectively.  More study results on other driving elements can be found on the project website. 

\subsection{Summary of Analysis} 
When using cosine similarity, smaller distances between vectors will yield a measurement closer to 1, while larger distances will be closer to -1. 
For projected distance, we observe that cosine similarity between feature vectors produces a consistent trend with classification confidence for the ``collision'' prediction, whereas FID and SSIM show inconsistent trends in capturing the same correlation. In level 1, where the change in the projected distance over an image sequence is the least, we expect that a safe situation far away from a vehicle will remain safe since the projected distance barely changes over time. Likewise, in level 4, which features the largest change in projected distance over time, we observe that the cosine similarity between model-level representations drastically decreases, showing change in model decision making correlating to collision confidence. 

Gradient results can be interpreted as the difference in learning perception between raw image data and gradient/saliency maps. For cosine similarity, we expect the similarity scores across sequences with similar collision confidences to be consistent. The bottom section of Table~\ref{tab:ablation-gradient} shows the normalized standard deviation measurements across all sequences based on method and metric. For most cases, cosine similarity appears to be the most consistent metric in terms of retaining relevance to decision confidence. 

% In different scenarios representing diverse spatio-temporal elements, we see that model-level perception between base data and saliency/gradient maps are very close per cosine similarity. Table \ref{tab:scenarios} shows that, for multiple test cases involving different driving scenarios, the combination of saliency maps and the spatio-temporal features account for around 78\% contribution in the latent representations of the trained network. With this, we further conjecture that transferring these latent representations to train another network on a different domain dataset, tunes the network to emphasize on the spatio-temporal features, and thus enhance the transfer learning mechanism to incorporate the temporal features in addition to the standard spatial features transfer learning.  Next, we describe our method for improving generalization of transfer learning based on our hypothesis.   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Gradient results also tell us that despite major color differences between reference and target images, cosine similarity still remains significant, since a similarity of 1 indicates complete equality on the feature vector space. Additionally, the cosine similarity stays consistent in standard deviation (and likewise variance) when classification confidence of ``collision'' is constant across different sequences of images. {\em This result suggests that cosine similarity considers semantic representation of the image more than merely pixel-level differences}. 

% \vspace*{0.5em}
% \noindent
% \subsection{Significance of Visual Driving Elements  }
% Since cosine similarity measures the closeness in orientation of features vectors, higher values of cosine similarity indicate that the network-level representations of data are closer. When we choose reference and target images to feed through the CNN+LSTM network, we control the change in chosen factors over time by choosing the reference and target images, and observe change in their representations within the classifier itself. When the feature-level representations in the classifier are far apart, the cosine similarity computed will be lower. Thus, one interpretation is that high cosine similarity measurements (closer to 1) can be correlated with greater significance in decision making when the reference image has high classification confidence. 

% Table~\ref{tab:scenarios} shows mean cosine similarities where reference images are unprocessed training images and target images are resulting saliency maps, as well as representative of specific driving scenarios. Here, mean cosine similarity is a significant value, which suggests that the feature-level representation of raw data is similar to the feature-level representation of corresponding saliency maps. 

% To calculate the values in the table, we first choose sequences of data which are representative of specific driving scenarios. Then, to create the target images, we create both saliency maps and gradient maps from the original unprocessed images and use them jointly to compute cosine similarity between sequences. The reference image sequences consist of 15 original unprocessed driving images from CARLA. The target sequences consist of the corresponding processed images. For example, in the `agent with nearby vehicle' scenario, the target sequences consist of 8 saliency maps, 2 gradient maps, and 5 images with background information outside of road edges subtracted. Mean cosine similarity is computed for every scenario in this fashion. The high mean cosine similarity suggests that subtracting background information from images will only slightly alter feature-level representations in learning. 

% To study the significance of the spatio-temporal features, our test sequence involves a combination of saliency maps, image gradients as well as custom test datasets we create to study the factors like projected distance, agent's orientation, optical flow and dynamic obstacles. For example, in 'agent with nearby vehicle' scenarios, our test data sequence of 15 frames include saliency maps of the first eight sequence frames, two gradient maps of the next couple of frames in sequence, and apply background subtraction on the rest of the sequence frames, essentially to include the coherence of projected distance of nearby vehicles on the road as well as the other temporal factors and exclude the background noise. We extract the lstm hidden state representations for this test case and find the cosine similarity with the reference sequence (unprocessed image sequence of the test case). We perform this experiment for multiple test cases for different scenarios including agents moving with nearby vehicles, agent moving on empty roads, agent turning and agent stationary with dynamic obstacles moving around the agent. 

      

% In projected distance, the reference images would show a vehicle traveling straight, with the nearest vehicle in sight a large distance away. Level 1 through 4 would show distances between vehicles becoming smaller, which eventually influences the confidence in the classifier labeling ``safe''. These changes are reflected in the intermediary layers of the CNN+LSTM network, which we extract during evaluation on each sequence of images. 

% For vehicle rotation, we obtain test images through preprocessing to emphasize changing elements, where canny edge detection is applied along with manual background erasure in order to track the rotation of the vehicle in reference to a stationary object in the scene. The reference images represent the unprocessed images, while levels indicate an incremental increase in rotation angles. 

% Grayscale gradients are emphasized through image gradient processing techniques such as Grad-CAM and Vanilla backpropagation. The purpose of this element is to find change over pixel level values over time. The reference image we use is a raw image with no preprocessing or transformations applied. Since there is no such way to vary the intensity in applying these gradient techniques, we show three example sequences to show the measurements of cosine similarity when pixel-level values are completely altered. In addition, we include ground-truth values of classification confidence on the "collision" decision. We use confidence as a reference for expectations in behavior across varying intensities of driving components and trends in similarity. 

% We use cosine similarity between word embeddings for studying the similarities between latent state embeddings in layers of the LSTM. By studying these hidden states, we hope to find insight into the affect of each factor in the classification decision. We choose cosine similarity over metrics like Euclidean or Manhattan distance cosine similarity avoids the Curse of Dimensionality for vectors with high-dimension, similarly to comparisons in semantic text similarity.

% We use a cosine similarity matrix to find the distance between the hidden state representation vectors for the reference input and the controlled noise induced test input.The cosine similarity is calculated by the equation ~\ref{eq:1} where   $x$ and $y$ are the LSTM hidden state representation vectors from reference input and noise induced input respectively.

% \begin{equation}
%  \label{eq:1}
%  similarity(x,y) =  \frac{x \cdot y}{||x|| ||y||}
% \end{equation}

% Additionally, we calculate the similarity using Pearson $\rho$ and Distance $dCor$ correlations in equations ~\ref{eq:2} and ~\ref{eq:3} respectively. 

% \begin{equation}
%  \label{eq:2}
%  \rho(x,y) =  \frac{cov(x,y)}{\sqrt{\sigma_x \sigma_y}} 
% \end{equation}

% \begin{equation}
%  \label{eq:3}
%  dCor(x,y) =  \frac{dCov(x,y)}{\sqrt{dVar(x) dVar(x)}} 
% \end{equation}

% Pearson coefficient is found by dividing the covariance of random variables $X$ and $Y$ by the standard deviations of $X$ and $Y$, whereas distance correlation is calculated by dividing the distance covariance $dCor$ by the product of their distance standard deviations. More details on the calculation of the distance correlation can be found on the project website. 

% Factors are isolated by choosing sequences of images in which all information is semantically constant except for the factor we are studying. For example, in studying the significance of projected distance from nearby vehicles, we isolate sequences in which the only information changing is the distance between vehicles (i.e. no rotational elements or optical flows, changes in lighting, new obstacles, etc). Then, we select a reference sequence as the baseline of comparison, in which the "safe" classification is confident and clear to the classifier. The framework for collecting these hidden state representations can be found in figure ~\ref{fig:control-system}. Continuing the example with projected distance, we show examples of reference and test sequences below, in figures ~\ref{fig:example-ref-sequence} and ~\ref{fig:example-test-sequence}. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=8cm]{imgs/example-reference-sequence.png}
%     \caption{Example reference sequence for projected distance between vehicles. In terms of projected distance between vehicles, this sequence shows a case of high confidence where the classifier would label this sequence as "safe". }
%     \label{fig:example-ref-sequence}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=8cm]{imgs/example-test-sequence.png}
%     \caption{Example test sequence for projected distance between vehicles. Test sequences are chosen at intervals where the factor is represented at varying intensities; in this example, the nearby car is very close. In the ablation study, we analyze test sequences at varying projected distances to study the significance of each factor in the "safe" and "dangerous" binary classification task.}
%     \label{fig:example-test-sequence}
% \end{figure} The ablation study setup pictured in figure ~\ref{fig:control-system} involves five stages.

% We design a neural network architecture which learns the temporal features and the spatial features across multiple frames and combines them to have the continuity perspective of the vehicle driving process. The network is trained on the end-to-end task of  predicting whether the set of frames or the environmental states lead to a collision or does not lead to a collision.
% %We induce noise in the sequence of test frames to focus on the global spatio-temporal feature we aim to examine. Hence, we create custom test datasets to study each of the features as follows.
% We extract these components by selectively choosing which data to feed through the network. By choosing data representative of the factor we want to examine, we can study the changes in the hidden state representation of the LSTM during the learning process as change in the factor is observed across frames. The following factors are studied:
%     \begin{itemize}
%         \item Projected distance: Our test sets, where each set is a sequence of frames, include scenarios with nearby vehicle/vehicles at a distance from the our self driving car
%         \item Optical flow:  Our test sets include scenarios where we extract saliency maps on our reference test frames. 
%         \item Rotational component: Our test sets include scenarios where upon extracting saliency maps, we choose few references like the lane edges and lane dividers etc. in the sequence of frames and do a background subtraction of all the other objects/elements in the sequence of frames.
%         \item Gradient information: \textbf{Laura: Notes: RGB gradient depends on the environmental lighting (brightness, saturation, etc. ). We may be getting an inconsistent percentage because of this. For grayscale, it will still persist. But, adding 3 channels will affect the color gradient. } We use the Gradient-weighted Class Activation Mapping technique \cite{selvaraju2017grad} to produce the coarse localization maps of the sequence of frames highlighting the important regions and the temporal features across the frames. Our test cases include these localisation maps as the input test sequence for the model.
%         \item Dynamic obstacles: Our test cases include obstacles like pedestrians moving from left to right and vice versa at the crossing as well as vehicles coming from the opposite lane. We do a background subtraction of all the other elements and features in the sequence of frames.  
%     \end{itemize}
% We pass these custom test dataset into our trained model an obtain the prediction results. % which is not our focus. 
% In this stage, we focus on extracting the hidden state representation vectors of the LSTM layer of our model for the custom test inputs we pass. This is the first hidden state representation vector. 
% Then, we pass the test datasets from which we derived our custom test dataset into our trained model.  These are the test datasets on which we performed manual background subtraction in stage 3 to create our custom dataset. These test datasets also includes the "safe" scenarios or the sequence of frames which predict to not to lead to collision. Upon passing these test sets, we obtain the second state representation vectors. 
% Finally, we use a cosine similarity matrix between the two state representation vectors obtained from previous two stages to determine the quantitative measures of influence of the global spatio-temporal feature vector on the learning outcome.

% The cosine similarities between sequences represent how different latent representations are when the differences in the sequences are isolated to one semantic target factor. Higher similarities correlate with a higher significance in the decision making process for a "safe" classification. Below, the show the results of the ablation study for several factors: 1) projected distance from nearby vehicles, 2) rotational component/optical flow, and 3) dynamic obstacles.

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c c}
%     \toprule
%         Sequence & z & Cosine & Pearson & Distance & FID & SSIM \\ 
%         \midrule
%         Reference & 92 & 1 & 1 & 1 & 0 & 1\\ 
%         Level1 & 65 & 0.8812 & 0.8815 & 0.8815 & 158.326 & 0.511\\
%         Level2 & 45 & 0.7806 & 0.7814 & 0.7813 & 237.496 & 0.439\\
%         Level3 & 18 & 0.35 & 0.356 & - & 258.921 & 0.513\\
%         Level4 & 4 & 0.2859 & 0.2843 & 0.2842 & 237.108 & 0.415\\
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative study of the \textbf{projected distance} weightage in collision avoidance behaviour.Closer the nearby vehicle in a driving scenario, more the weightage of the projected distance in the AI decision making. We extract the spatio-temporal feature embeddings of a reference scenario which has far-off projected distance of nearby vehicle and calculate its distance from the embeddings from test cases with lesser projected distance of the nearby vehicles. We observe that as the projected distance of nearby vehicles decreases, the spatio-temporal embeddings become less similar to the 'safe' reference scenario}
    
%     %Measurement of \textbf{projected distance z (m)} using similarity between hidden LSTM states. In a collision recognition binary classification task, we expect from human experience that distance to nearby vehicles plays a large role in evaluating the safety of a situation. Here, smaller gaps between nearby vehicles greatly affects the state of the LSTM in decision making, showing that projected distance quantitatively plays a significant role in decision making.}
%     \label{tab:ablation-distance}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=8cm]{imgs/metric-trend.png}
%     \caption{\textbf{Line plot of image similarity measurements over increasing classifier confidence.} Here, the results from table~\ref{tab:ablation-distance} are plotted. The y axis denotes the normalized values measured by the metric, where normalization is calculated with the max value of measured values. The x axis represents the classifier confidence of a "collision" label. In order to observe trends fairly against FID, a distance metric, the values measured from similarity metrics were inverted. Among the three metrics considered, cosine similarity, colored in blue, is the only to show a consistent non-decreasing trend as collision confidence increases. }
%     \label{fig:metric-trend}
% \end{figure}


\iffalse
\begin{table}[h!]
    \centering
    \begin{tabular}{c|c c c c c c}
    \toprule
        Sequence & Angle & Cosine & Pearson & Distance & FID & SSIM\\
        \midrule
        Reference & 0 & 1 & 1 & 1 & 0 & 1\\ 
        Level1 & 5-20 & 0.8003 & 0.7995 & 0.7995 & 379.445 & 0.0911\\
        Level2 & 30-40 & 0.4286 & 0.4280 & 0.4280 & 454.313 & 0.0860\\
        Level3 & 50-60 & 0.7317 & 0.7293 & 0.7293 & 446.039 & 0.0770\\
        Level4 & 70-80 & 0.7811 & 0.7809 & 0.7809 & 396.968 & 0.0813\\
    \bottomrule
    \end{tabular}
    \caption{Measurement of \textbf{optical flow} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }
    \label{tab:ablation-optflow}
\end{table}
\fi

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c c}
%     \toprule
%         Sequence & Angle & Cosine & Pearson & Distance & FID & SSIM\\
%         \midrule
%         Reference1 & 5-20 & 1 & 1 & 1 & 0 & 1\\ 
%         Level1 & 5-20 & 0.159 & 0.156 & 0.156 & \\
%         Reference2 & 30-40 & 1 & 1 & 1 & 0 & 1\\ 
%         Level2 & 30-40 & 0.291 & 0.291 & 0.291 \\
%         Reference3 & 50-60 & 1 & 1 & 1 & 0 & 1\\ 
%         Level3 & 50-60 & 0.320 & 0.330 & 0.330 & \\
%         Reference4 & 70-80 & 1 & 1 & 1 & 0 & 1\\ 
%         Level4 & 70-80 & 0.345 & 0.345 & 0.345 & \\
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative study of the \textbf{Rotational component} weightage in collision avoidance behaviour.More the lane curves/turns in divider edges etc., more the steering angle change required and hence more the rotational component weightage. We combine canny edge detection with image processing techniques to extract lane curves and edges as our test cases from our references.Note that the test cases contain the segmented rotational information of the references. We extract the spatio-temporal feature embeddings of reference scenarios and calculate its similarity from the respective test case embeddings. We observe that in cases with more steering angles, the embeddings of the test case are more similar to the references indicating the increasing rotational elements weightage.}
    
%     %Measurement of \textbf{rotational factors (steering angle)} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }
%     \label{tab:ablation-optflow}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c}
%     \toprule
%         Seq & Angle & Cosine & FID & SSIM & Confidence(\%)\\
%         \midrule
%         %Ref & - & \textbf{1} & 0 & 1 & -\\ 
%         Level1 & 0-20 & \textbf{0.159} & 346.224 & 0.1217 & 1.2\\
%         % Reference2 & 30-40 & 1 & 0 & 1\\ 
%         Level2 & 30-40 & \textbf{0.291} & 428.305 & 0.1172 & 10.2 \\
%         % Reference3 & 50-60 & 1 & 0 & 1\\ 
%         Level3 & 50-60 & \textbf{0.320} & 427.043 & 0.1035 & 15.6\\
%         % Reference4 & 70-80 & 1 & 0 & 1\\ 
%         Level4 & 70-80 & \textbf{0.345} & 433.655 & 0.1022 & 19.4\\
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative study of cosine similarity trends over changes in the \textbf{rotational component} of the vehicle. Measurements are taken over chronological sequences of images; the angle represents the range of rotation over each sequence. As confidence in ``collision'' classification increases, we expect a steady linear increase in cosine similarity measurements. Intuitively, the confidence in collision also increases as rotation angles become sharper. While FID shows generally increasing results, but is inconsistent; SSIM shows an entirely inverted trend. }
    
%     %More the lane curves/turns in divider edges etc., more the steering angle change required and hence more the rotational component weightage. We observe that as the steering angle increases, the cosine weightage of the rotational component and the collision probablity increases linearly and the slope of the linear relationship is small     }
    
%     %Measurement of \textbf{rotational factors (steering angle)} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }
%     \label{tab:ablation-rotation}
%     \vspace*{-1.5em}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c c}
%     \toprule
%         Sequence & Angle & Cosine & Pearson & Distance & FID & SSIM\\
%         \midrule
%         Reference1 & 5-20 & 1 & 1 & 1 & 0 & 1\\ 
%         Level1 & 5-20 & 0.321 & 0.315 & 0.315 \\
%         Reference2 & 30-40 & 1 & 1 & 1 & 0 & 1\\ 
%         Level2 & 30-40 & 0.364 & 0.364 & 0.364 \\
%         Reference3 & 50-60 & 1 & 1 & 1 & 0 & 1\\ 
%         Level3 & 50-60 & 0.424 & 0.414 & 0.414 \\
%         Reference4 & 70-80 & 1 & 1 & 1 & 0 & 1\\ 
%         Level4 & 70-80 & 0.481 & 0.472 & 0.473 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Measurement of \textbf{coherence of optical flow and rotational component} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }
%     \label{tab:ablation-optflow-coherence}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c}
%     \toprule
%         Seq & Angle & \textbf{Cosine} & FID & SSIM  & Confidence(\%)\\
%         \midrule
%         %Ref & - & \textbf{1} & 0 & 1 &  -\\  
%         Level1 & 0-20 & \textbf{0.461} & 390.94 & 0.00064 & 1.2 \\
%         % Reference2 & 30-40 & 1 & 0 & 1\\ 
%         Level2 & 30-40 & \textbf{0.498} & 429.751 & 0.00191 & 1.2 \\
%         % Reference3 & 50-60 & 1 & 0 & 1\\ 
%         Level3 & 50-60 & \textbf{0.499} & 426.341 & 0.00237  & 1.2\\
%         % Reference4 & 70-80 & 1 & 0 & 1\\ 
%         Level4 & 70-80 & \textbf{0.529} & 457.358 & 0.00805 & 1.3\\
%         \midrule
%         $\widetilde{\sigma}$ & - & \textbf{0.0560} & 0.0639 & 1.0139 & 0.0408\\
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative study cosine similarity trends over changes in \textbf{coherence of rotational component and optical flow}. Since rotation and optical flow are closely related, we study their joint contribution for decision making. For a constantly low classification confidence for ``collision'', the cosine similarity stays constant with values significant in relation to the max value of 1. As observed with other elements, FID and SSIM show inconsistent trends relative to changes in confidence as well as failure to reflect similarities between reference sequences and level 1-4 sequences, where all sequences represent ``safe'' classifications. Normalized standard deviation $\widetilde{\sigma}$ (standard deviation divided by mean) is also calculated to show the stability of the metric over constant classification confidence. }
    
    %An increase in vehicle turn is usually associated with a decrease in velocity, and a hence the rotational component and optical flow combined usually have the weightage in fixed range. We observe that the cosine weightage of the coherence vary about a mean of around 49 percent and there exist a constant relationship to the collision probablity}
    
%Measurement of \textbf{coherence of optical flow and rotational component} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }%
%     \label{tab:ablation-optflow-coherence}
%     \vspace*{-3em}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c}
%     \toprule
%         Sequence & Angle & Cosine & Pearson & Distance \\
%         \midrule
%         Reference & 0 & 1 & 1 & 1\\ 
%         Level1 & 5-20 & 0.321 & 0.315 & 0.315 \\
%         Level2 & 30-40 & 0.364 & 0.364 & 0.364 \\
%         Level3 & 50-60 & 0.424 & 0.414 & 0.414 \\
%         Level4 & 70-80 & 0.481 & 0.472 & 0.473 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Measurement of \textbf{dynamic obstacles} using similarity between hidden LSTM states. In this table, we observe that a changing rotation causes latent state to change significantly compared to the state where the steering angle is at 0 degrees. }
%     \label{tab:ablation-optflow-coherence}
% \end{table}

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c c}
%     \toprule
%         Sequence & Technique & Cosine & Pearson & Distance & FID & SSIM\\
%         \midrule
%         Ref & None & 1 & 1 & 1 & 0 & 1\\ 
%         1 & Grad-CAM  & 0.6355 & 0.6254 & 0.6255 \\
%         1 & Vanilla & 0.6357 & 0.6356 & 0.6356 \\
%         2 & Grad-CAM  & 0.5688 & 0.5688 & 0.5687 \\
%         2 & Vanilla & 0.6240 & 0.6234 & 0.6235 \\
%         3 & Grad-CAM  & 0.6320 & 0.6321 & 0.6321 \\
%         3 & Vanilla & 0.6330 & 0.6335 & 0.63322\\
%     \bottomrule
%     \end{tabular}
%     \caption{Measurement of \textbf{grayscale gradients} using similarity between hidden LSTM states.  For gradient extraction and analysis, we applied color transformations to the reference using Grad-CAM and Vanilla (Grayscale) backpropagation. \textbf{TODO: Generate more results here with possibly Yu's color gradient levels for HSV, to simulate varying weather/lighting conditions. RGB may be too impractical (?)}}
%     \label{tab:ablation-optflow}
% \end{table}


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c c c c c}
%     \toprule
%         Seq & Velocity & \textbf{Cosine} & FID & SSIM & Confidence(\%)\\
%         \midrule
%         %Ref & - & \textbf{1} & 0 & 1\\ 
%         1 & 2   & \textbf{0.11503} & 418.494 & 0.1371 & 3.4\\
%         2 & 3  & \textbf{0.1210} & 393.076 & 0.1506 & 3.5\\
%         3 & 4  & \textbf{0.1307} & 538.536 & 0.14435 & 3.2\\
%         \midrule
%         $\widetilde{\sigma}$ & - & 0.0647 & 0.1726 & \textbf{0.0469} & 0.0454 \\
%         %3 & 5 & \textbf{0.1563} & &\\
%     \bottomrule
%     \end{tabular}
%     \caption{Quantitative study of cosine similarity trends in relation to \textbf{dynamic obstacles}. Velocity is measured in units of pixels per frame, i.e. the actual speed of objects across image representations rather than actual speed relative to the simulation world. 
%     %weightage in collision avoidance behaviour. 
%     We consider the cases where the dynamic obstacles are traveling in the opposite lane and the pedestrians are moving on the cross street when the agent is stationary. Dynamic obstacles do not show an obvious relationship between any of the three metrics, velocity, or classification confidence of ``collision''. In terms of normalized standard deviation $\widetilde{\sigma}$, the most closely related metric is SSIM. }
    
    
    
    
%     %We observe that the weightage is within the range of 10-15 percent with slight increase  with increasing velocity of the dynamic obstacle and a constant relation with the collision probability}
    
%     %An increase in vehicle turn is usually associated with a decrease in velocity, and a hence the rotational component and optical flow combined usually have the weightage in fixed range . We use canny edge detection to extract edges information of our test cases from our references.Note that the test cases contain the combined rotational and optical flow information segmented from the references. We extract the spatio-temporal feature embeddings of reference scenarios and calculate its similarity from the respective test case embeddings. We observe that the weightage vary around a mean of around 49}
%     \label{tab:ablation-dynamicobstacles}
%     \vspace*{-3em}
% \end{table}







%We use our abalation study methodology \ref{} to quatify the mean weightage of coherence of these spatio temporal features in the
